Holistic Cube Analysis: A Query Framework for Data Insights

Many data insight questions can be viewed as searching in a large space of tables and finding important ones, where the notion of importance is defined in some adhoc user defined manner. This paper presents Holistic Cube Analysis (HoCA), a framework that augments the capabilities of relational queries for such problems. HoCA first augments the relational data model and introduces a new data type AbstractCube, defined as a function which maps a region-features pair to a relational table (a region is a tuple which specifies values of a set of dimensions). AbstractCube provides a logical form of data, and HoCA operators are cube-to-cube transformations. We describe two basic but fundamental HoCA operators, cube crawling and cube join (with many possible extensions). Cube crawling explores a region space, and outputs a cube that maps regions to signal vectors. Cube join, in turn, is critical for composition, allowing one to join information from different cubes for deeper analysis. Cube crawling introduces two novel programming features, (programmable) Region Analysis Models (RAMs) and Multi-Model Crawling. Crucially, RAM has a notion of population features, which allows one to go beyond only analyzing local features at a region, and program region-population analysis that compares region and population features, capturing a large class of importance notions. HoCA has a rich algorithmic space, such as optimizing crawling and join performance, and physical design of cubes. We have implemented and deployed HoCA at Google. Our early HoCA offering has attracted more than 30 teams building applications with it, across a diverse spectrum of fields including system monitoring, experimentation analysis, and business intelligence. For many applications, HoCA empowers novel and powerful analyses, such as instances of recurrent crawling, which are challenging to achieve otherwise.

==> Makefile <==
### Makefile --- 

TARGETS = paper

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files
	rm -f *.bbl

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.bbl *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls



==> alt_intro.tex <==
Data analytics and business intelligence tools have traditionally focused on delivering insights by filtering, categorizing, and aggregating data to identify trends.
In such a setting, the analyst first selects the appropriate filters and categories of interest;
they then use tools to efficiently process the data; and present the aggregated data in some visually meaningful way so that the trends are easy to distil and view.
In the above description the analyst knows what they are looking for and can express it in a succinct way so the tools can render the results efficiently and appropriately.
In that sense, the process is arguably forward: from hypothesis, to insights supporting the hypothesis, through the processing of data.
What is equally---if not more---important, however, is being able to explain outputs without any prior hypothesis.
Such an attribution exercise is a backward process: given an outlier or some surprising result, what are the parts of the input that can justify its presence?
And how can we turn that justification into an insight?  

Figure~\ref{fig:example-hoca-questions} presents two such insight questions:
In Figure~\ref{fig:most-important-contributros-from-base-table} we observe a top-level CostPerClick
change, and we want to know the slices that are the root causes for the change; whereas in
Figure~\ref{fig:most-important-outliers-from-base-table} we want to identify the ``most interesting'' outliers among a large space of slices.
To support such analysis using existing OLAP tools, traditionally powered by SQL, one needs to construct
complex workflows that are customized for the case at hand and oftentimes use esoteric and highly specific toolchains that are external to a relational engine.
While there exists limited support for data explanation (e.g.,~\cite{AKSGXSASM21, ABDGMNRS18, WDM15, WM13})
there is no generic way to slice and analyze the space of inputs in order to rank them in terms of importance of likelihood of being root causes for an observed behavior.
Worse yet, any customized way resorts to changing representations and interfacing with external data models (\textit{e.g.}, data frames, table-valued functions, \textit{etc.}).
The results are predictable: loss of performance, increased engineering effort, higher maintenance costs, excessive need for manual tuning, creation of data and knowledge silos---to name but a few.
Clearly, we need to do better; and we can.

Our solution is \textbf{Ho}listic \textbf{C}ube \textbf{A}nalysis (\textbf{HoCA}):
a framework for systematically augmenting the capabilities of
relational queries to efficiently and effectively support and deliver data insights.
Unlike previous efforts we follow a first-principles approach:
HoCA  augments the relational data model by defining a new type called AbstractCube.
The key enabling property of AbstractCube is that it is not a typical data type, but it is actually a \emph{function} from table subsets, which we call RegionFeatures, to relational tables.
Intuitively, RegionFeatures partition tabular space by filtering on attributes (regions) and extracting computed values (features) and are represented as points; therefore, given the coordinates of a RegionFeature we can identify the combination of filters that have created it and the values it has computed.
AbstractCube provides a \emph{logical form} of data,
where how these functions are encoded is hidden from upper abstractions such as HoCA operators.
We only know that the application of the function is possible and type-safe; that the function is invertible: once we observe the output of the function we can identify the RegionFeature that was used as its argument.
We can then follow the backward analysis process we mentioned earlier: from outputs to the inputs that contributed to their presence.

Figure~\ref{fig:hoca-cube-func} gives a visualization of HoCA cube logically as a function.
Function-as-data modeling allows us to encode \emph{two} structures in \emph{one} data object:
(a) space of non-uniform tables on the co-domain of the function, and
(b) a uniform region space on the domain of the function.
Both structures are fundamental if one's goal is to search the region space for insights.
With abstract cubes, we can then design operators that are cube-to-cube 
transformations. (i.e., \emph{higher order}, function-to-function transformations)
These operators can be composed where HoCA cubes flow in between.
Figure~\ref{fig:hoca-operators} visualizes the HoCA operator concept.

\begin{figure*}[htb]
  \centering
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{
      figures/most-important-contributors-from-base-table.png}
    \caption{
      Finding important contributors to
      CostPerClick change, starting from a base table.
      While seemingly simple, a principled answer
      requires applying the AumannShapley method,
      see Section~\ref{sec:programmability}
      and Section~\ref{sec:density-model-derivation}
      for details.
    }
    \label{fig:most-important-contributros-from-base-table}
  \end{subfigure}
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{
    figures/most-important-outliers-from-base-table.png}
    \caption{Finding important timeseries outliers,
      starting from a base table: Given a large space of slices,
      what are \emph{important} timeseries outliers one must pay attention to?
    }
    \label{fig:most-important-outliers-from-base-table}
  \end{subfigure}\quad
  \caption{\small
    Many data insights problems can be viewed as:
    Given a \emph{space of tables} (often called slices)
    that are aggregated at different granularity,
    find interesting, or most attention-worthy slices
    (where these notions often need to be defined in an ad-hoc manner).
    Currently, to perform such analysis, analysts often need to build complex workflows to generate the tables,
    and then analyze them using advanced statistical and ranking techniques.
    By contrast, Figure~\ref{fig:hoca-programs-for-example-questions}
    shows that one can answer these questions using succinct HoCA programs.
  }
  \label{fig:example-hoca-questions}
\end{figure*}

\begin{figure*}[htb]
  \centering
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{
    figures/hoca-cube-func.png}
    \caption{A HoCA cube: A function mapping region-features to
    relational tables. It provides a logical form of the data. In particular,
    HoCA programmers do not need to care about how the function mapping is computed.
    For example, a HoCA cube may not be generated by typical projection-groupby-aggregation
    using SQL.
    }
    \label{fig:hoca-cube-func}
  \end{subfigure}\quad
  \begin{subfigure}{0.50\textwidth}
    \centering
    \includegraphics[width=\linewidth]{
      figures/hoca-paradigm.png}
    \caption{
      A HoCA operator: A cube-to-cube transformation (i.e., a higher-order function).
      In this figure we illustrated a ``cube crawling'' operator: We examine a region subspace,
      and for each region we analyze timeseries features and detect interesting outliers.
      The ``function-as-data'' modeling of HoCA cubes is critical for composition here:
      Because the output is also a HoCA cube, we can apply further HoCA operators to the
      output cube (even though it may not be a projection-groupby-aggregation one).
      This gives rise to constructions such as Recurrent Cube Crawling (see Section~\ref{sec:compositions}).
    }
    \label{fig:hoca-operators}
  \end{subfigure}
  \caption{\small
    \textbf{The HoCA paradigm}.
  }
  \label{fig:hoca-paradigm}
\end{figure*}

We describe two basic, but fundamental, HoCA operators:
\emph{Cube crawling} and \emph{cube join} (there are many more possibilities devising
more useful HoCA operators and extend the algebraic framework, which we discuss in
Section~\ref{sec:discussions}). Cube crawling introduces a enumeration-type operator,
which allows one to scan regions in a subspace, and extracts useful signals and put
results into an output cube. Cube join, in turn, melds two input cubes into one,
by joining tables from two region-features spaces (see Figure~\ref{fig:cube-join}
for a visualization of the concept). Cube join is critical for \emph{composition},
since it allows one to join information from different cubes for deeper analysis,
and it shows up in some of our most complex HoCA programs
(e.g., Recurrent Cube Crawling in Section~\ref{sec:recurrent-crawling}).

To solve a rich family of insight analytic problems,
we design cube crawling with two novel \emph{programming} features:
{\bf (1)} {\em Region Analysis Models (RAMs)},
which allows one to program and organize adhoc analysis on a set of data features
into a module. This enables easy integration with advanced analytic techniques
(such as timeseries outlier detection (\cite{PyBSTS}),
causal inference (\cite{BGKRS15}),
differentiable programming (\cite{jax_2018_github}),
which goes much beyond previous works (e.g.~\cite{AKSGXSASM21}).
To this end, crawling RAM has a notion of \emph{population data},
which allows one to capture complex notions of ``region importance''.
{\bf (2)} {\em  Multi-model crawling}, which allows one to apply multiple models,
potentially on {\em different} feature sets, during crawling.
Multi-model crawling significantly broadens the scope of analytic questions
one can answer with a single crawl.

\begin{figure*}[htb]
  \centering
  \begin{subfigure}{0.40\textwidth}
    \centering
    \includegraphics[width=\linewidth]{
    figures/hoca-program-most-important-outliers.png}
    \caption{A HoCA program for finding important timeseries outliers.
    `importance\_score' is based on both region and population features. 
    }
    \label{fig:hoca-program-most-important-outliers}
  \end{subfigure}\quad\quad\quad
  \begin{subfigure}{0.40\textwidth}
    \centering
    \includegraphics[width=\linewidth]{
      figures/hoca-program-most-important-contributors.png}
    \caption{A HoCA program for finding important contributors to CostPerClick change.
      `aumann\_shapley\_attribution' is based on both region and population features.}
    \label{fig:hoca-program-most-important-contributors}
  \end{subfigure}
  \caption{\small
    HoCA programs that use cube crawling to answer the analytic questions raised in
    Figure~\ref{fig:example-hoca-questions}. In both cases, we analyze features from
    \emph{both the region and the entire population},
    which is holistic compared to analyzing region features alone.
  }
  \label{fig:hoca-programs-for-example-questions}
\end{figure*}

Together, these abstractions are designed to greatly simplify the insights analysis workflows aforementioned,
and also go beyond in capturing even more complex data insights problems.
Figure~\ref{fig:hoca-programs-for-example-questions} shows two HoCA programs that
answered formal versions of the two analytic questions in Figure~\ref{fig:example-hoca-questions}.
Each program only consists of basically three statements: Initializes a cube,
initializes an appropriate region analysis model, and then performs a cube crawling.
HoCA programmers can also construct more complex HoCA programs by composing HoCA operators,
together with standard relational constructions,
since HoCA abstractions are compatible with standard relational constructions.

We have implemented and deployed HoCA in a large search-engine company.
HoCA poses a rich algorithmic design space, such as optimizing
crawling performance (leveraging region space structure),
optimizing cube join performance (local v.s. global join),
and physical design of cubes (i.e., encoding of functions).
We briefly describe several implementations of HoCA based on different foundations
(an in-house distributed relational query engine (\cite{F1Query}),
and also Apache Beam (\cite{PythonBeam})),
and evaluate their main performance characteristics.

HoCA has found a variety of applications in system monitoring, experimentation analysis,
and business intelligence. In most of our applications, our users are system builders,
who use our new query framework to build data-insights systems.
Even in this early stage, there have been more than 30 teams directly dependent
on our codebase. In several applications, an interesting finding is that users had already built
adhoc solutions that can be captured by HoCA, and migrating to HoCA 
not only significantly simplified these constructions, but also improved performance and scalability,
and enabled new functionalities. In several Business Intelligence (BI) applications,
HoCA enabled fast build of novel data insights functionalities,
such as discovering important anomalies, trends, attributions, and correlations,
within a highly complex region space. These BI applications have helped generate
significant revenue uplift.

\textbf{HoCA vs. OLAP}.
Both HoCA and OLAP talked about ``cubes'', which indeed share some similarities.
For example, OLAP cubes can provide \emph{encoding} of HoCA cubes,
by providing mapping functionality from region-features to a relational table.
A first major difference, however, is that HoCA and OLAP examine
\emph{entirely different analytic questions}.
To this end, OLAP operators (e.g. drill-down, roll-up, etc.)
provide analytic capabilities in the \emph{forward} direction,
where users can leverage OLAP operators to perform an iterative, but manual,
slice-and-dice analysis to find data insights. HoCA, however, provides operators to analyze
the cube in the \emph{backward} direction to \emph{automate} searching for data insights.
For example in the CostPerClick attribution case described in Figure~\ref{fig:most-important-contributros-from-base-table},
HoCA starts with the \emph{top-level} CostPerClick change,
and the analysis deconstructs the metric and search for the regions
that are major contributors to this change.
This difference in analytic questions induces vastly different considerations of
the cube design: In HoCA, cubes are designed to be a \emph{logical form} of data,
and HoCA operators are about higher-order, cube-to-cube transformations. These operators
can be composed in a HoCA program, where HoCA cubes flow in between. 
OLAP cubes are, on the other hand, designed for entire languages (e.g.~\cite{MDX})
for forward cube analytic capabilities. OLAP cubes are monolithic data objects,
and there is little sense of OLAP cubes explicitly flowing between operators.
To this end, HoCA provides novel \emph{programming experiences} and \emph{constructions},
such as Region Analysis Model programming, cube join, and recurrent cube crawling,
which are all beyond OLAP considerations.
A more detailed comparison can be found in Section~\ref{sec:olapcomparison}.

\textbf{Paper organization}.
Section~\ref{sec:preliminaries} presents necessary background.
Section~\ref{sec:framework} presents the HoCA framework of
HoCA cubes and operators.
Section~\ref{sec:power} gives various examples of programming
using HoCA to find data insights.
Section~\ref{sec:considerations} discusses important algorithmic considerations.
Section~\ref{sec:impl-eval} presents our current implementation of HoCA and its evaluations on several data sets.
We also briefly overview real-world HoCA applications.
Section~\ref{sec:discussions} discusses related work and future avenues,
and finally Section~\ref{sec:conclusion} concludes.

==> preliminaries.tex <==
\textbf{A simple relation to facilitate the discussion}.
To facilitate the discussion, we consider the following simple relation as a
``base relation'', over which we construct data cubes,
and then apply cube analysis operators over the cubes.

\begin{table}[htb]
  \centering\small
    \begin{tabular}{l|l|l|l}
      \toprule
      \textbf{Device} & \textbf{Browser} & \textbf{Date} & \textbf{Revenue} \\ \hline\hline
      Pixel 5a & Chrome & 2022-01-01 & 100 \\\hline
      iPhone 13 & Safari & 2022-01-01 & 200 \\\hline
      Surface Go 2 & Chrome & 2022-01-01 & 1000 \\\hline
      ... & ... & ... & ... \\\hline
      \bottomrule
    \end{tabular}
  \caption[]{\small A relation $\bfB$ for facilitating the discussion.
    In this relation, we have four columns \textbf{Device}, \textbf{Browser},
    \textbf{Date}, and \textbf{Revenue}. For example, the first tuple
    says that the revenue is \$100 on Chrome on a Pixel 5a device on 2022-01-01.
  }
  \label{tab:base-relation}
\end{table}

\textbf{Dimensions and measures}.
As in OLAP cubes, we distinguish two kinds of columns: Dimensions and measures.
Dimensions are columns that induce ``groups'' w.r.t. which we aggregate,
while measures are the objects to aggregate.
For example, we can define a measure `TotalRevenue', as an aggregation `SUM(Revenue)'.
Then for the `Device' dimension, we can aggregate
the Revenue over all devices to get the total revenue.
We can also consider any specific value of device, and aggregate
Revenue to get total revenue for that device.
In this paper, for simplicity, dimensions are synonymous to attributes,
and measures are synonymous to metrics.

\textbf{Region}\label{def:region}.
A region is an \emph{assignment} of \emph{some}
(could be a proper subset) dimensions.
For example, (Device=`Pixel 5a') is a region.
(Device=`Pixel 5a', Browser=`Chrome') is another region.
For a region $\gamma$ and a dimension $d$,
we use $\gamma[d]$ to denote the value of $d$ takes in $\gamma$.
We use $\dim(\gamma)$ to denote all the dimensions in the region.
We call the number of dimensions in the region the \emph{degree} of the region.
For example, (Device=`Pixel 5a') is a degree-1 region, and
(Device=`Pixel 5a', Browser=`Chrome') is a degree-2 region.
% yaqizhang Should we also discuss degree-0 region here?

\textbf{Filtering a relation by a region}.
If $\bfB$ is a relation, we use $\bfB[\gamma]$ to denote
the set of tuples in $\gamma$ induced by a filtering:
For any $d$, $\bfB[\gamma]$ takes value $\gamma[d]$ for dimension $d$.
In SQL, this simply corresponds to a WHERE clause on $\bfB$.
For example, $\bfB[\text{Device=`Pixel 5a'}]$ considers tuples
where Device is `Pixel 5a'.

\textbf{Features}.
A feature is a dimension or a measure.
For example, `Device' is a (dimension) feature,
and `TotalRevenue' is a (measure) feature.
We use $D$ to denote a set of dimension (attribute) features,
and $M$ to denote a set of measure (metric) features.
For example we can have $D = [\text{`Device', `Browser'}]$, and
$M = [\text{`TotalRevenue'}]$.
